Reward Conditioned Neural Movement Primitives for Population Based Variational Policy Optimization

The aim of this paper is to study the reward based policy exploration problem in a supervised learning approach and enable robots to form complex movement trajectories in challenging reward settings and search spaces. For this, the experience of the robot, which can be bootstrapped from demonstrated trajectories, is used to train a novel Neural Processes-based deep network that samples from its latent space and generates the required trajectories given desired rewards. Our framework can generate progressively improved trajectories by sampling them from high reward landscapes, increasing the reward gradually. Variational inference is used to create a stochastic latent space to sample varying trajectories in generating population of trajectories given target rewards. We benefit from Evolutionary Strategies and propose a novel crossover operation, which is applied in the self-organized latent space of the individual policies, allowing blending of the individuals that might address different factors in the reward function. Using a number of tasks that require sequential reaching to multiple points or passing through gaps between objects, we showed that our method provides stable learning progress and significant sample efficiency compared to a number of state-of-the-art robotic reinforcement learning methods. Finally, we show the real-world suitability of our method through real robot execution involving obstacle avoidance.

==> deleted.tex <==
From Intro:
A recent approach, \cite{schmidhuber2020reinforcement} proposed to map rewards to actions to make reinforcement learning more similar to supervised learning. In this work, we bring the same vision into movement primitives framework with a more sophisticated representation learning and exploration process. We use an improved version of Conditional Neural Movement Primitives \cite{Seker2019} as our base framework.

\utku{Our framework with reward conditioning only does not generate distinct enough trajectories due to the well-formed latent space, so we used the crossover and mutation operations to facilitate exploration. Mutation operation is performed by adding a smooth Gaussian noise on top of trajectories.}


\tuluhan{The main difference between RL and LfD is that the agent receives error? \utku{Solda bir soru işareti var} signals coming from   in supervised learning but receives evaluation? signals in reinforcement learning. Many approaches combined LfD with RL to benefit from both learning types to facilitate sample-efficient learning \cite{dulac2019challenges}. Expert demonstrations are used to limit the large search space in which RL looks for a solution to manageable volumes by providing  well performing initial experiences to the algorithm \cite{hester2018deep, vecerik2019practical}. A recent approach, \cite{schmidhuber2020reinforcement} proposed to map rewards to actions to make reinforcement learning more similar to supervised learning. In this work, we bring the same vision into movement primitives framework with a more sophisticated representation learning and exploration process. }

%(Utku:Learning  from  Demonstration  (LfD)  [1]  has  beenwidely used to teach robots complex skills including objectmanipulation  [2],  [3],  [4],  [5],  [6].  LfD  assumes  that  acertain  amount  of  demonstrations  have  been  collected  insome way (kinesthetic, coordinates, video etc.) and that thesedemonstrations  are  optimal  or  sufficiently  close  to  beingoptimal.  These  methods  easily  achieve  success  on  staticenvironments,  learning  methods  that  are  based  on  dynamicsystems  [7],  statistical  modeling  [8]  and  their  combination[9], [?] have gained popularity in recent years. In changingenvironments, learning and adjusting behaviour appropriatelyis  desired.  Dynamic  Movement  Primitives  (DMPs)  encodethe demonstrated trajectory as a set of differential equations,implementing a spring-mass-damper system extended with anon-linear function which also includes a point attractor forreaching a specified end-point of a trajectory. Due to the theirlinear  spring  system,  they  can  generate  motion  trajectoriesthat  can  directly  adapt  to  novel  initial  and  goal  positions.Encountered with novel situations, the model parameters ofthe DMP can be adjusted using reinforcement learning [10],[11]. While DMPs generate deterministic trajectories, Prob-abilistic  Movement  Primitives  (ProMPs)  [12]  can  encode  adistribution  of  trajectories  and  generate  stochastic  policies.Conditional  Neural  Movement  Primitives  (CNMP)  [?]  alsoencode trajectory distributions. Different from ProMPs, CN-MPs allow learning non-linear relationship between environ-ment  parameters  and  complex  action  trajectories  and  allowcomplex  conditioning,  i.e.  conditioned  by  high-dimensionalvariables and parameters. While CNMPs allow learning from demonstrations  only,  its  extension,  namely  ACNMPs  allowefficient  policy  improvement  in  novel  environments  andeffective  skill  transfer  between  different  agents.  This  wasachieved through exploiting the latent representation learnedby the underlying Conditional Neural Process (CNP) model,and  simultaneous  training  of  the  model  with  supervisedlearning (SL) for acquiring the demonstrated trajectories andvia  RL  for  new  trajectory  discovery.  However  ACNMPsfail short of finding motion trajectories that are significantlydifferent from the demonstrations in sample efficient way.)


%\tuluhan{ Our model starts with demonstrations or random trajectories with corresponding reward values. Using these trajectories, it forms its latent presentation according to described LfD framework above \ref{fig:generalfigure}.I. Afterwards, using the obtained best reward value ($r'$) the model samples more trajectories, these trajectories are gone through crossover, mutation and PD controller blocks and evaluated by the reward function before they are added to replay buffer \ref{fig:generalfigure}.II. After the replay buffer received new generation trajectories, the model reforms its latent representation and repeats this procedure until convergence
\tuluhan{
In movement primitives framework, trajectories are defined as $\tau = \{x_t\}_{t=0,...,T}$ where $x_t$ can be joint positions or Cartesian positions. The trajectory distribution $p(\tau)$ can be conditioned on a set of observations ($O = \{x_t\}_{t \in \{0,...T,\}} $) such as via-points or external task parameters ($\gamma$): $p(\tau|O,\gamma)$. As described above CNMP's encoder network can produce trajectory representations w.r.t. observations and task parameters and its decoder network can produce a full trajectory from this representation. However, this representation is deterministic and it is not practical to take samples from this latent space. Since we want to capture the trajectory distribution in latent space, we model the latent space as a Gaussian distribution $p(z) = N(0, I)$ and optimize our network using variational inference like $\beta$-Variational Auto-Encoders ($\beta$-VAE) (referans). The log-likelihood of trajectory is composed of log-likelihoods of individual data points: $\log p_\theta(\tau|O,\gamma) \quad & = \sum\limits_{t=1}^T \log p_\theta(x_t|O,\gamma)$
The log-likelihood can be expressed as:
\begin{equation}
\begin{aligned}
\log p_\theta(x_t|O,\gamma) \quad & = \mathbb{E}_{q_\phi(z|O,\gamma)}[\log p_\theta(x_t|O,\gamma)] \\
\quad & = \mathbb{E}_{q_\phi(z|O,\gamma)}[\log \frac{ p_\theta(x_t,z|O,\gamma)}{q_\phi(z|O,\gamma)}] \\
\quad & - \mathbb{E}_{q_\phi(z|O,\gamma)}[\log \frac{ q_\phi(z|O,\gamma)}{p_\theta(z|x_t,O,\gamma)}]
\end{aligned}
\end{equation}

The first term before the minus is the evidence lower bound (ELBO) $\mathcal{L}(\theta,\phi;x_t,z,O,\gamma)$ and the second term is a KL divergence term, which is non-negative. Therefore, ELBO is a lower bound on the likelihood of data. ELBO can also be expressed as:
\begin{equation}
\label{objective}
\begin{aligned}
\mathcal{L}(\theta,\phi;x_t,z,O,\gamma,\beta)  = \mathbb{E}_{q_\phi(z|O,\gamma)}[\log p_\theta(x_t|z,O,\gamma)] \\
- \beta D_{KL} \left(q_\phi(z|O,\gamma) \middle\| p_\theta(z|O,\gamma) \right)
\end{aligned}
\end{equation}

}


\utku{CNMP \cite{sekerconditional} is a deep neural architecture based on Conditional Neural Processes \cite{CNP}, able to learn multi-modal nonlinear relationships between high dimensional sensorimotor data and complex movement trajectories from expert demonstrations. The network learns a conditional distribution, and is able to be conditioned on time alone to yield an average trajectory based on the learned representation; or together with sensorimotor data or external parameters, able to follow user specified conditions to output a trajectory or react robustly to changes in an online setting during execution. During training, sampled observations from an expert demonstration are encoded to a latent space via an encoder network $E$, and then averaged to yield a single representation which is then queried with a different point from the demonstration. The query network $Q$ generates from this representation a Gaussian with \mu and \sigma parameters for that point. Training is done for all given expert demonstrations, and during testing, the network generates a trajectory which is compliant with the observations provided as the conditions. The formulation is as follows:
\begin{equation}
\label{eqn:cnp}
\begin{aligned}
\mu_{q}, \sigma_{q} = Q_{\theta} \left(x_{q} \oplus  \frac{\Sigma_{i}^{n}E_{\phi}((x_{i}, y_{i}))}{n} \right)
\end{aligned}
\end{equation}

where $x_{q}$ is the target query for which we want the predictions, $\{(x_{i}, y_{i})\}_{i=0}^{n}$ are the sampled observations, \oplus denotes concatenation, \phi and \theta are parameters of the encoder and query networks respectively.
}



\utku{In Genetic-Gated Networks \cite{chang2018genetic}, a chromosome vector which mutates and is subject to crossover is employed, controlling the gating choices of the network. Genetic algorithm is used for optimization of this vector, on populations of generated chromosome vectors based on their attained rewards. This portion constitutes the exploration phase. In the next phase, the chromosome vector representing the best choice is taken and the resulting network is subjected to gradient based optimization, and the process repeats. Their argument is that this two-phase process allows hopping over the loss surface with different chromosome vectors for decent exploration and converging to a local optima better than other explored local optima.}

\utku{In  Genetic Policy Optimization \cite{gangwani2017policy}, the approach is a genetic algorithm utilizing both imitation learning and deep reinforcement learning within. Crossover step is done not on the parameter space but on state space. Two parent policy networks are subjected to crossover via applying imitation learning on their offspring in order to generate a state space distribution similar to its parents'. Mutation operation is done by policy gradient methods, updated with high variance gradients; supplying enough diversity for exploration.}

\utku{Recently, ES have been used first as a better scalable alternative to RL  \cite{salimans2017evolution}, \cite{such2017deep}, and later approaches using them together came forward. While ES approaches are quick for small number of parameters, they suffer from exponential complexity for large number of parameters. RL methods, while being able to handle a large number of parameters, are harder to optimize and take longer wall clock time to train. So using them together yields a best of both worlds solution. RL is used to reduce the parameter search space, and ES finds a solution in a sample efficient manner in this reduced space; leading to solutions which are both sample efficient and able to work for a large number of parameters \cite{}. \cite{}, instead of sampling from the high-dimensional input space, performs sampling from the latent space.}

\utku{In \cite{wang2020instance}, Natural ES is applied directly on network parameters, however the process is regulated by instance weighting, and the learning problem is tackled for dynamic environments; unlike previous approaches. Instance weighting depends on two metrics: instance novelty, which is how different the instance is from the optimum point of the network's solution of the previous environment; and instance quality is the performance of the instance in the current environment. Instance weighting enables both exploration to novel regions and regions with high returns. Incremental improvements enable the algorithm to retain some information from the previous environment, helping the adaptation to new environments.}


\utku{In \cite{conti2018improving}, similar to \cite{wang2020instance} instance novelty and quality are taken into account while optimizing the parameters of a network. In this approach, robustness against deceptive rewards is investigated and it is shown that the ES approach performs better on such tasks than RL, since it encourages different behaviours more, avoiding the local optima that RL gets stuck on in the end.}

Additionally, our approach encourages exploration in states with high reward by conditioning on higher rewards, similar to a directed exploration. To improve exploration, we used all experiences of the robot, good and bad, by adding two random trajectories in addition to the best performing trajectory of the current generation to the replay buffer, which serves as the selection process. ACNMP is trained on each generation enough to learn the improvements from it, then the process continues with a new generation.


% Bu buraya gelmeyebilir.
\utku{Our approach uses crossover on both the replay buffer which is from the previous experiences of earlier generations, and on the current generation which results in faster learning.}

\utku{In \cite{wang2020instance}, Natural ES is applied directly on network parameters, however the process is regulated by instance weighting, and the learning problem is tackled for dynamic environments; unlike previous approaches. Instance weighting depends on two metrics: instance novelty, which is how different the instance is from the optimum point of the network's solution of the previous environment; and instance quality is the performance of the instance in the current environment. Instance weighting enables both exploration to novel regions and regions with high returns. Incremental improvements enable the algorithm to retain some information from the previous environment, helping the adaptation to new environments.}



\utku{ERL \cite{khadka2018evolution}, PDERL \cite{bodnar2019proximal} , and CEM-RL \cite{pourchot2018cem} are similar approaches combining ES and DDPG, but CEM-RL appears to be superior to ERL in sample efficiency and performance on the MuJoCo benchmark tasks. The authors explain this by noting that in ERL, the RL agent is injected to the population only from time to time whereas in CEM-RL gradient steps are applied in each iteration. PDERL performs better than CEM-RL in some benchmarks, and the authors note that while the approaches are similar in many ways; PDERL can benefit from gradient free optimization while CEM-RL cannot.}

However the process is regulated by instance weighting \utku{which assigns higher weights to instances that contain more new knowledge}, and the learning problem is tackled for dynamic environments; unlike previous approaches. Instance weighting here depends on two metrics: instance novelty, which is how different the instance is from the optimum point of the network's solution of the previous environment; and instance quality is the performance of the instance in the current environment. Instance weighting enables both exploration to novel regions and regions with high returns.


\tuluhan{
Silinecek:
- Supervised learning is more stable than reinforcement learning because we optimize parameters for the objective; to learn, to generalize and to reproduce data. However, in reinforcement learning, we obtain partial information, rewards, from the environment but the true policy is not given to us as data. This partial information can be noisy and unsatisfactory so the learning process can be oscillatory or inefficient. Therefore, \cite{schmidhuber2020reinforcement} proposed to map rewards to actions to make reinforcement learning more similar to supervised learning. In this work, we bring the same vision into the movement primitives framework with a more sophisticated representation learning and exploration process. 

- We want to condition trajectories with reward values and to express trajectory distribution in latent space, so that we can sample trajectories that give high rewards. Therefore, we need variational inference and construct a similar architecture to Conditional Variational Auto-Encoders \cite{Sohn2015}.

- Mutation operation takes place in the task space by adding smooth Gaussian noise to trajectories because latent space is well-formed to represent the trajectories in replay buffer and therefore, it is hard to sample trajectories different from the existing ones by using latent space only. 

- Crossover operation takes place because of the same problem and we try to increase variation in trajectories by activating different representations at different time steps. We also think that bad trajectories may possess good sub-parts that receive rewards from different portions. Combination of these sub-parts in a new trajectory accelerates the learning. 
%What is this
- Instead of incremental desired value, sampling with the best reward with high variance produces similar effect, incremental desired value decreased the stability of learning when I tried. If the increment value is well optimized as hyper-parameter, I think it may work.

- 

Our contribution can be summarized as follows:

- Incorporating supervised learning's advantages to reinforcement learning in movement primitives framework. 
- Distribution in latent space for CNMPs as opposed to deterministic latent space.
- Benefit from genetic algorithms to accelerate the learning.
}

The challenges are as follows: 
\begin{itemize}
    \item The challenge that requires variational inference
    \item The challenge that requires mutation operation in latent space.
    \item The challenge that requires combining multiple solutions that address/solve different sub-problems in the task, receive rewards from different portions. Small changes do not suffice, therefore combining the solutions is required.
    \item The challenge that requires conditioning the system with incremental desired values. 
\end{itemize}

Our contributions to solve these challenges are as follows:
\begin{itemize}
    \item Variational inference (opposed to deterministic inference) in the latent space. This is achieved by...
    \item Gaussian noise in the latent space. This is achieved by.. Is formulated as mutation operation in the latent representation of the skill to be improved. 
    \item Considering that different parts of the motion trajectories address different sub-problems, generate new skills by temporal blending of the latent representations of different solutions. As underlying CNPs encode the full trajectory, this can be possible. 
    \item Formalize the framework as a population based algorithm where multiple individual solutions are formed, and mutation and crossover operations are applied to generate better
    \item Condition the skill in order to generate higher rewards. As the reward based conditioning requires extrapolation capability, i.e. generating significantly different trajectories for novel rewards, incremental approach is applied.
\end{itemize}


$x_t,t,z,O,r,\beta$

Different modes of reward landscapes.  

Sparse reward. 


\ahmet{
Tahminen yazıyorum bunları da, burayı daha iyi bağlamak lazım. Şu an üstte problemleri veriyoruz ama, bizim framework'ün niye bu problemleri çözdüğünü onpoint sunmuyoruz gibi geldi. Aklıma geleni yazdım. Çok iyi değil ama fikir verir belki.

In this work, we propose Reward Conditioned Neural Movement Primitives that tackles these problem. Our framework improves sample diversity by using good and bad experience alike for learning a reward conditioned policy mapping function. This allow our framework to learn about the reward landscape, preventing it from generating samples from previously explored low reward landscapes. Our framework can generate progressively improved trajectories by sampling them from high reward landscapes, increasing the reward gradually. By further utilizing mutation and crossover operation in exploration, our system can quickly deal with complexity of the search space and converge to a diverse solution pool. We compared our method to the state of the art DREPS model and acquired better performance with over 5x sample efficiency.}

We propose a model that generates motion trajectories conditioned with desired rewards. The system tries to increase the reward gradually, by generating progressively improved trajectories. Furthermore, in order to deal with the complexity of the search space, operations similar to mutation and crossover are applied. In particular, the solution pool is diversified by applying Gaussian noise in the latent representation of the underlying neural network and crossover is applied to different individual solutions. 

 Sample efficiency is critical for RL when applied in the real-world since experimenting with the real robot takes time, and resources. If done in an inefficient manner also risks wearing out or endangering the robot.There RL algorithms may have reduced performance, or have lower sample efficiency on tasks which have many local optima. Potential causes for that include not sampling with enough diversity, and also while policy search algorithms attempt to optimize for the best returns, they do not use all the information that is available from the samples; such as bad actions or bad states, thus repeating the same mistakes which ends up reducing sample efficiency. This is undesired but acceptable in simulation experiments, however in a real-world learning setting may be problematic. Certain actions for a robot may lead to potentially dangerous outcomes and the expected behaviour would be to learn from bad experiences and to not repeat previous mistakes. Our proposition is to learn a more complete approximation of the policy by utilizing the experiences of the robot better.

Intro sıralamasında söyle bir degisiklik yaptım, paragrafın az basını degistirdim.

The main difference between RL and LfD is that in LfD the agent receives supervision signals based on skill similarity, while in RL the agent receives supervision signals based on task reward. Many approaches combine LfD with RL  {to benefit from both approaches} to facilitate sample-efficient learning \cite{dulac2019challenges}. Expert demonstrations are used to limit the large search space in which RL looks for a solution to manageable volumes by providing  well performing initial experiences to the algorithm \cite{hester2018deep, vecerik2019practical}

Sample efficiency is critical for RL when applied in the real-world since experimenting with the real robot takes time, and resources. If done in an inefficient manner, this also risks wearing out or endangering the robot. Therefore, LfD approaches are widely used, where LfD  provides  expert  knowledge  about  the  task  execution, effectively giving a prior to constrained policy search so that a solution can be found faster and safer.

\ahmet{

  We condition the experienced trajectories with the corresponding rewards to fully train our model in a supervised learning setting. Reward conditioning also incorporates samples with undesired outcomes into policy mapping function. Unlike \cite{schmidhuber2020reinforcement}, our framework predicts trajectories as whole, allowing {it to optimize them}{optimization} for long horizon rewards?(Uzun vadeli yüksek reward RL'de ne olarak geçiyor.). % Bu cümle wordy oldu, düzeltmek lazım.

 % Tuluhan sizin method'a göre düzeltebilirsin.
We observed that this operation accelerates the learning, because sub-parts of undesired trajectories, which receive rewards from different portions, could possibly be combined. The Mutation operation is used to diversify the solution pool by applying Gaussian noise in the task space. This further accelerates the learning progress since neural networks are not very good at generating too distinct trajectories from the observed ones.  


%Mutation operation takes place by adding a smooth Gaussian noise on top of trajectories, because latent space is well-formed to represent the trajectories in the data set and therefore, it is hard to sample trajectories different from the existing ones with a fixed decoder by using latent space only. % Bu cümleyi farklı yazmak lazım, burada sanki method'un geri kalanını disliyor gibi oluyor. Mutation'ı crossover'ı tamamlayıcı olarak şey yapmak belki.
}

\tuluhan{




 
 
 In the first experiment, the advantages of stochastic sampling in latent space are displayed in comparison with \cite{Seker2019}, in the second experiment, the stability of using supervised learning even for RL problems is portrayed opposed to a recent state of art policy gradient algorithm on top of movement primitives \cite{Akbulut2020}. In the last experiment, we showed our models' sample efficiency in a real world multi-modal problem against 2 baseline policy search algorithms \cite{colome2017dual,peters2010}.
  
  

}

\tuluhan{
We use an improved version of Conditional Neural Movement Primitives \cite{Seker2019} as our base framework. Here, we conditioned the experienced trajectories with the corresponding rewards to fully train our model in a supervised learning setting. Reward conditioning also incorporates samples with undesired outcomes into policy mapping function. Furthermore, we benefit from Genetic Algorithms (GA) and variational inference to explore the environment efficiently. Variational inference is used to create a stochastic latent space to sample varying trajectories conditioned on rewards in a similar architecture with Conditional Variational Auto-Encoders \cite{Sohn2015}. Crossover operation is used to increase diversity of trajectories by activating sampled representations in different time steps. We observed that this operation accelerates the learning, because sub-parts of undesired trajectories, which receive rewards from different portions, could possibly be combined. Mutation operation takes place by adding a smooth Gaussian noise on top of trajectories, because latent space is well-formed to represent the trajectories in the data set and therefore, it is hard to sample trajectories different from the existing ones with a fixed decoder by using latent space only.
}

%Instance weighting is shown to enable exploration to both novel regions and regions with high returns. Incremental improvements enable the algorithm to retain some information from the previous environment, helping the adaptation to new environments. \cite{conti2018improving} also takes novelty and quality into account while optimizing the parameters of a network. In this approach, robustness against deceptive rewards is investigated. Deceptive rewards are the reward functions of an environment when greedy progress towards high rewards, combined with low variance exploration leads to a sub-optimal policy. \utku{They showed that their ES approach performs better on dynamic tasks designed to be deceptive compared to certain baseline RL, ES and meta learning approaches, since it encourages different behaviours more through novelty search \cite{lehman2011novelty}, avoiding convergence to the local optima in the end.}

==> todo.tex <==


- fig.1'e robot execution'dan reward geldigi eklenecek
- fig.1'de NMP yerine RC-NMG yazilacak.
- fig.1'de n mutation operations degil, m mutation operations yazilacak
- fig.1'de replay buffer (I), Reward-Conditioned Neural Movement Generation (RC-NMG) (II), population generation conditioning with r_max (bu eksik) (III), cross-over (IV), mutation (V), PD-control (VI), eklenecek


